Outlier Suppression+: Accurate quantization of large language models by equivalent and optimal shifting and scaling

Post-training quantization~(PTQ) of transformer language models faces significant challenges due to the existence of detrimental outliers in activations. We observe that these outliers are concentrated in specific channels and are asymmetric across channels. To address this issue, we propose the Outlier Suppression+~(OS+) framework, which contains the channel-wise shifting for asymmetry and channel-wise scaling for concentration. We show that these operations can be seamlessly migrated into subsequent modules while maintaining equivalence. Second, we propose a fast and stable scheme to calculate effective shifting and scaling values. The channel-wise shifting aligns the center of each channel for removal of outlier asymmetry. The channel-wise scaling quantitatively evaluates changes brought by migration and quantization for better quantization burden balance. We validate our OS+ under both standard and fine-grained quantization settings with models including BERT, OPT, BLOOM, BLOOMZ, and LLaMA. Comprehensive results across various tasks demonstrate the superiority of our approach. Especially, with standard quantization, OS+ can achieve near-floating-point performance on both small models and large language models on 8-bit and 6-bit. Besides, we establish a new state-of-the-art for 4-bit BERT with 15.5\% improvement. Our code is available at \url{https://github.com/ModelTC/Outlier_Suppression_Plus}.

==> tables/bloom.tex <==
\begin{table}[b!]
\vspace{-1em}
      \begin{adjustbox}{valign=t,max width=\linewidth}
      \begin{tabular}{llccccc}\toprule 
         Method & Bits & HellaSwag & LAMBADA & PIQA & Winogrande \\ 
         \hline
         BLOOM-176B & FP16  & 55.9 & 67.7 & 78.8 & 70.3 \\
         \hline
         \hspace{0.5em}ZeroQuant$^\clubsuit$ & INT8* & 54.8 & 67.8 & 76.0 & 69.4\\ 
         \hspace{0.5em}SmoothQuant &INT8* & 54.1 & \bf{69.2} & 77.7 & 68.6\\
         \hspace{0.5em}Ours  & INT8* & \bf{55.2} &  68.0 & \bf{78.4} & \bf{69.8}\\ 
         \hline
         \hspace{0.5em}ZeroQuant$^\clubsuit$ & INT6 & 30.5 & 7.5 & 61.2 & 52.0 \\ 
         \hspace{0.5em}SmoothQuant &INT6 & 52.1 & 60.2 & 76.7 & 67.6\\ 
         \hspace{0.5em}Ours  & INT6 & \bf{54.8} & \bf{69.2} & \bf{78.1} & \bf{70.3}\\
         \hline
         BLOOMZ-176B & FP16  & 57.1 & 67.8 & 80.6 & 72.5 \\
         \hline
         \hspace{0.5em}ZeroQuant$^\clubsuit$ & INT8* & 56.3 & 67.6 & 79.1 & 70.9\\ 
         \hspace{0.5em}SmoothQuant &INT8* & 56.3 & 68.7 &  79.7 & 70.8\\
         \hspace{0.5em}Ours  & INT8* & \bf{56.7} & \bf{68.8}& \bf{79.9} & \bf{71.3}\\ 
         \hline
         \hspace{0.5em}ZeroQuant$^\clubsuit$ & INT6 & 28.2 & 1.4 & 54.0 & 49.6 \\ 
         \hspace{0.5em}SmoothQuant & INT6 & 55.0 & 65.2 & \bf 80.0 & 69.9\\ 
         \hspace{0.5em}Ours  & INT6 & \bf{56.4} & \bf{69.2} & 79.9 & \bf{70.6} \\
        \bottomrule
    \end{tabular}  
    \end{adjustbox}
    \caption{Quantization results in terms of accuracy.}
    \label{tab_ptq_bloom}
\end{table}


==> tables/fine-grained_old.tex <==
\begin{table}[ht]
    \centering
    
    \begin{adjustbox}{max width=\textwidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{clcccccccc}
        \toprule
          \bf Model & \bf Method &  \textbf{PIQA} & \textbf{Winogrande} & \textbf{HellaSwag} & \textbf{WikiText2} \\
        \midrule
        & \bf FP16 & 77.37 & 66.93 & 72.99 & 9.41\\
        \cdashline{2-6}
        & \bf INT6 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ & \\
        LLaMA-1 & \hspace{0.5em}OS+ & 77.53 & & & 9.58\\
        \cdashline{2-6}
        7B & \bf INT4 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ \\
        & \hspace{0.5em}OS+ \\
    \midrule
        & \bf FP16 & 79.05 & 70.09 & 76.22 & 8.22\\
        \cdashline{2-6} 
        & \bf INT6 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ & \\
        LLaMA-1 & \hspace{0.5em}OS+ &  \\
        \cdashline{2-6}
        13B & \bf INT4 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ \\
        & \hspace{0.5em}OS+ \\
    \midrule
        & \bf FP16 & 80.09 & 72.77 & 79.21 & 6.10 \\
        \cdashline{2-6}
        & \bf INT6 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ & \\
        LLaMA-1 & \hspace{0.5em}OS+ & \\
        \cdashline{2-6}
        30B & \bf INT4 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ \\
        & \hspace{0.5em}OS+ \\
    \midrule
        & \bf FP16 & 80.85 & 77.11 & 80.73 & 4.94\\
        \cdashline{2-6}
        & \bf INT6 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ & \\
        LLaMA-1 & \hspace{0.5em}OS+ & \\
        \cdashline{2-6}
        65B & \bf INT4 \\
        & \hspace{0.5em}MinMax & \\
        & \hspace{0.5em}SQ \\
        & \hspace{0.5em}OS+ \\
    \end{tabular}
    \end{adjustbox}
    % }
    \caption{PTQ performance of BERT-base models. MNLI and STS-B report the combined score. \textbf{Avg.} indicates the averaged results of 8 tasks on GLUE benchmark (details in \autoref{supp_bert_base_ptq}). $*$ means per-tensor quantization for weight. OS indicates Outlier Suppression for short.}
    \label{tab_bert_ptq_narrow}
\end{table}
